TEMPO: Prompt-based Generative Pre-trained Transformer for Time Series Forecasting

The past decade has witnessed significant advances in time series modeling with deep learning. While achieving state-of-the-art results, the best-performing architectures vary highly across applications and domains. Meanwhile, for natural language processing, the Generative Pre-trained Transformer (GPT) has demonstrated impressive performance via training one general-purpose model across various textual datasets. It is intriguing to explore whether GPT-type architectures can be effective for time series, capturing the intrinsic dynamic attributes and leading to significant accuracy improvements. In this paper, we propose a novel framework, TEMPO, that can effectively learn time series representations. We focus on utilizing two essential inductive biases of the time series task for pre-trained models: (i) decomposition of the complex interaction between trend, seasonal and residual components; and (ii) introducing the design of prompts to facilitate distribution adaptation in different types of time series. TEMPO expands the capability for dynamically modeling real-world temporal phenomena from data within diverse domains. Our experiments demonstrate the superior performance of TEMPO over state-of-the-art methods on zero shot setting for a number of time series benchmark datasets. This performance gain is observed not only in scenarios involving previously unseen datasets but also in scenarios with multi-modal inputs. This compelling finding highlights TEMPO's potential to constitute a foundational model-building framework.

==> table_align/table4_abalation_short.tex <==
\begin{wraptable}{l}{0.6\textwidth}
    \caption{Ablation study on  TEMPO. }
    \label{tab:long_term_ablation_study_final}
    
    \begin{small}
    \scalebox{0.8}{
    \renewcommand{\arraystretch}{1.5}
    \centering
    \setlength\tabcolsep{3pt}
    \hspace{20pt}
    \begin{tabular}{c|c|c|c|c|c}
    \hline\hline
     ~ & ~ & TEMPO & w/o Dec & w/o Pro & w/o Dec Loss  \\ \cline{3-6}
     ~ & ~ & MSE/MAE & MSE/MAE & MSE/MAE & MSE/MAE \\ \hline\hline
        ECL & Avg. & \textbf{0.216}/\textbf{0.308} & 0.228/0.319 & 0.219/0.313 & 0.225/0.322  \\ 
         \hline
        Ettm1 & Avg. & \textbf{0.501}/\textbf{0.458} & 0.575/0.481 & 0.506/0.466 & 0.515/0.475  \\ \hline\hline
        
        % ~ & ~ & \multicolumn{2}{c|}{TEMPO} & \multirow{2}{*}{GPT4TS} & \multirow{2}{*}{w/o Pro} & \multirow{2}{*}{w/o Dec Loss} \\ \cline{3-4}
        % ~ & ~ & Hard&Pool &  & &  \\ \cline{3-7}
        % ~ & ~ & MSE/MAE & MSE/MAE & MSE/MAE & MSE/MAE & MSE/MAE \\ \hline\hline
        % \multirow{5}{*}{ECL} & 96 & \textbf{0.178}/\textbf{0.276}& \underline{0.18}/\textbf{0.276} & 0.189/0.286 & 0.185/\underline{0.281} & 0.191/0.293  \\ \cline{2-7}
        % ~ & 192 & \underline{0.198}/\textbf{0.293}& 0.204/0.307 & 0.206/0.302 & \textbf{0.196}/\underline{0.295} & 0.205/0.305  \\ \cline{2-7}
        % ~ & 336 & \textbf{0.209}/\textbf{0.309} & 0.236/0.326  & 0.232/0.324 & \underline{0.225}/\underline{0.318} & 0.243/0.337 \\ \cline{2-7}
        % ~ & 720 & 0.279/0.355 & \textbf{0.259}/\textbf{0.346} & \underline{0.262}/\underline{0.347} & 0.269/0.359 & \underline{0.262}/0.353  \\ \cline{2-7}
        % ~ & Avg & \textbf{0.216}/\textbf{0.308} & 0.22/0.314  & 0.222/0.315 & \underline{0.219}/\underline{0.313} & 0.225/0.322 \\ \hline\hline
        % \multirow{5}{*}{Ettm1} & 96 & 0.438/\underline{0.424} & \underline{0.43}/\textbf{0.412} & 0.486/0.438 & 0.452/0.431 & \textbf{0.428}/0.425  \\ \cline{2-7}
        % ~ & 192 & \textbf{0.461}/\textbf{0.432}& \underline{0.464}/\underline{0.443} & 0.516/0.461 & 0.47/0.45 & 0.494/0.463  \\ \cline{2-7}
        % ~ & 336 & \underline{0.515}/\underline{0.467} & \textbf{0.507}/\textbf{0.466}& 0.571/0.502 & 0.519/0.474 & 0.544/0.492  \\ \cline{2-7}
        % ~ & 720 & 0.591/\underline{0.509}& \underline{0.583}/\textbf{0.505}  & 0.646/0.54 & \textbf{0.582}/0.51 & 0.594/0.521 \\ \cline{2-7}
        % ~ & Avg & \underline{0.501}/\underline{0.458}& \textbf{0.496}/\textbf{0.457} & 0.555/0.485 & 0.506/0.466 & 0.515/0.475  \\ \hline\hline
        % \multirow{2}{*}{~} & \multirow{2}{*}{~} & TEMPO & GPT4TS & T54TS & Bert4TS & PatchTST \\ \cline{3-7}
        % ~ & ~ & MSE/MAE & MSE/MAE & MSE/MAE & MSE/MAE & MSE/MAE \\ \hline\hline
        %  \multirow{5}{*}{ECL} & 96 & \textbf{0.19}/\textbf{0.29} & 0.202/0.301 & \underline{0.199}/\underline{0.293} & 0.202/0.298 & 0.21/0.308 \\ \cline{2-7}
        % ~ & 192 & \textbf{0.211}/\textbf{0.31} & \underline{0.217}/0.313 & 0.238/0.337 & 0.227/0.321 & 0.223/\underline{0.312} \\ \cline{2-7}
        % ~ & 336 & \textbf{0.229}/\textbf{0.323} & 0.258/0.353 & 0.273/0.364 & \underline{0.256}/\underline{0.345} & 0.282/0.357 \\ \cline{2-7}
        % ~ & 720 & \textbf{0.375}/\textbf{0.444} & \underline{0.43}/\underline{0.475} & 0.455/0.49 & 0.442/0.479 & 0.606/0.561 \\ \cline{2-7}
        % ~ & Avg & \textbf{0.251}/\textbf{0.342} & \underline{0.277}/\underline{0.361} & 0.291/0.371 & 0.282/\underline{0.361} & 0.33/0.385 \\ \hline\hline
        % \multirow{5}{*}{Traffic} & 96 & \underline{0.56}/0.411 & 0.607/0.417 & \textbf{0.543}/\underline{0.408} & 0.591/0.423 & 0.577/\textbf{0.403} \\ \cline{2-7}
        % ~ & 192 & \textbf{0.575}/\underline{0.419} & 0.603/0.421 & \underline{0.594}/0.431 & 0.613/0.432 & 0.596/\textbf{0.411} \\ \cline{2-7}
        % ~ & 336 & \textbf{0.597}/\textbf{0.433} & \underline{0.63}/\underline{0.435} & 0.659/0.458 & 0.639/0.445 & 0.665/0.454 \\ \cline{2-7}
        % ~ & 720 & \underline{0.65}/\underline{0.452} & \textbf{0.643}/\textbf{0.439} & 0.69/0.49 & 0.744/0.496 & 0.802/0.501 \\ \cline{2-7}
        % ~ & Avg & \textbf{0.595}/\underline{0.429} & \underline{0.621}/\textbf{0.428} & 0.622/0.447 & 0.647/0.449 & 0.66/0.442 \\ \hline\hline
        % \multirow{5}{*}{Weather} & 96 & \textbf{0.217}/\textbf{0.268} & 0.288/0.31 & 0.252/0.288 & \underline{0.237}/0.288 & 0.249/\underline{0.285} \\ \cline{2-7}
        % ~ & 192 & \textbf{0.265}/\textbf{0.302} & 0.305/0.331 & 0.322/0.336 & 0.291/0.323 & \underline{0.277}/\underline{0.314} \\ \cline{2-7}
        % ~ & 336 & \underline{0.322}/\underline{0.342} & 0.338/0.353 & 0.346/0.358 & 0.335/0.354 & \textbf{0.311}/\textbf{0.341} \\ \cline{2-7}
        % ~ & 720 & 0.41/0.397 & \textbf{0.381}/\textbf{0.377} & 0.444/0.42 & 0.466/0.436 & \underline{0.385}/\underline{0.386} \\ \cline{2-7}
        % ~ & Avg & \textbf{0.304}/\textbf{0.327} & 0.328/0.343 & 0.341/0.351 & 0.332/0.35 & \underline{0.305}/\underline{0.331} \\ \hline\hline

        
    \end{tabular}
    }
\end{small}
\end{wraptable}


==> table_align/table4_ablation.tex <==
\begin{wraptable}{l}{0.6\textwidth}
    \caption{Ablation study on  MSE/MAE for
long-term forecasting with respect to prompt pool
and time series decomposition. The best results
are highlighted in bold.}
    \label{tab:long_term_ablation_study_final}
    
    \begin{small}
    \scalebox{0.8}{
    \renewcommand{\arraystretch}{1.5}
    \centering
    \setlength\tabcolsep{3pt}
    \hspace{20pt}
    \begin{tabular}{c|c|c|c|c|c}
    \hline\hline
    ~ & ~ & TEMPO & w/o Dec & w/o Pro & w/o Dec Loss  \\ \cline{3-6}
        ~ & ~ & MSE/MAE & MSE/MAE & MSE/MAE & MSE/MAE \\ \hline\hline
        \multirow{5}{*}{ECL} & 96 & \textbf{0.178}/\textbf{0.276} & 0.195/0.294 & \underline{0.185}/\underline{0.281} & 0.191/0.293  \\ \cline{2-6}
        ~ & 192 & \underline{0.198}/\textbf{0.293} & 0.210/0.301 & \textbf{0.196}/\underline{0.295} & 0.205/0.305  \\ \cline{2-6}
        ~ & 336 & \textbf{0.209}/\textbf{0.309} & 0.237/0.328 & \underline{0.225}/\underline{0.318} & 0.243/0.337  \\ \cline{2-6}
        ~ & 720 & 0.279/0.355 & 0.271/\textbf{0.351} & \underline{0.269}/0.359 & \textbf{0.262}/\underline{0.353}  \\ \cline{2-6}
        ~ & Avg & \textbf{0.216}/\textbf{0.308} & 0.228/0.319 & \underline{0.219}/\underline{0.313} & 0.225/0.322  \\ \hline\hline
        \multirow{5}{*}{Ettm1} & 96 & \underline{0.438}/\textbf{0.424} & 0.516/0.447 & 0.452/0.431 & \textbf{0.428}/\underline{0.425}  \\ \cline{2-6}
        ~ & 192 & \textbf{0.461}/\textbf{0.432} & 0.518/0.462 & \underline{0.47}/\underline{0.45} & 0.494/0.463  \\ \cline{2-6}
        ~ & 336 & \textbf{0.515}/\textbf{0.467} & 0.622/0.515 & \underline{0.519}/\underline{0.474} & 0.544/0.492  \\ \cline{2-6}
        ~ & 720 & \underline{0.591}/\textbf{0.509} & 0.644/0.50 & \textbf{0.582}/\underline{0.51} & 0.594/0.521  \\ \cline{2-6}
        ~ & Avg & \textbf{0.501}/\textbf{0.458} & 0.575/0.481 & \underline{0.506}/\underline{0.466} & 0.515/0.475  \\ \hline\hline
        
        % ~ & ~ & \multicolumn{2}{c|}{TEMPO} & \multirow{2}{*}{GPT4TS} & \multirow{2}{*}{w/o Pro} & \multirow{2}{*}{w/o Dec Loss} \\ \cline{3-4}
        % ~ & ~ & Hard&Pool &  & &  \\ \cline{3-7}
        % ~ & ~ & MSE/MAE & MSE/MAE & MSE/MAE & MSE/MAE & MSE/MAE \\ \hline\hline
        % \multirow{5}{*}{ECL} & 96 & \textbf{0.178}/\textbf{0.276}& \underline{0.18}/\textbf{0.276} & 0.189/0.286 & 0.185/\underline{0.281} & 0.191/0.293  \\ \cline{2-7}
        % ~ & 192 & \underline{0.198}/\textbf{0.293}& 0.204/0.307 & 0.206/0.302 & \textbf{0.196}/\underline{0.295} & 0.205/0.305  \\ \cline{2-7}
        % ~ & 336 & \textbf{0.209}/\textbf{0.309} & 0.236/0.326  & 0.232/0.324 & \underline{0.225}/\underline{0.318} & 0.243/0.337 \\ \cline{2-7}
        % ~ & 720 & 0.279/0.355 & \textbf{0.259}/\textbf{0.346} & \underline{0.262}/\underline{0.347} & 0.269/0.359 & \underline{0.262}/0.353  \\ \cline{2-7}
        % ~ & Avg & \textbf{0.216}/\textbf{0.308} & 0.22/0.314  & 0.222/0.315 & \underline{0.219}/\underline{0.313} & 0.225/0.322 \\ \hline\hline
        % \multirow{5}{*}{Ettm1} & 96 & 0.438/\underline{0.424} & \underline{0.43}/\textbf{0.412} & 0.486/0.438 & 0.452/0.431 & \textbf{0.428}/0.425  \\ \cline{2-7}
        % ~ & 192 & \textbf{0.461}/\textbf{0.432}& \underline{0.464}/\underline{0.443} & 0.516/0.461 & 0.47/0.45 & 0.494/0.463  \\ \cline{2-7}
        % ~ & 336 & \underline{0.515}/\underline{0.467} & \textbf{0.507}/\textbf{0.466}& 0.571/0.502 & 0.519/0.474 & 0.544/0.492  \\ \cline{2-7}
        % ~ & 720 & 0.591/\underline{0.509}& \underline{0.583}/\textbf{0.505}  & 0.646/0.54 & \textbf{0.582}/0.51 & 0.594/0.521 \\ \cline{2-7}
        % ~ & Avg & \underline{0.501}/\underline{0.458}& \textbf{0.496}/\textbf{0.457} & 0.555/0.485 & 0.506/0.466 & 0.515/0.475  \\ \hline\hline
        % \multirow{2}{*}{~} & \multirow{2}{*}{~} & TEMPO & GPT4TS & T54TS & Bert4TS & PatchTST \\ \cline{3-7}
        % ~ & ~ & MSE/MAE & MSE/MAE & MSE/MAE & MSE/MAE & MSE/MAE \\ \hline\hline
        %  \multirow{5}{*}{ECL} & 96 & \textbf{0.19}/\textbf{0.29} & 0.202/0.301 & \underline{0.199}/\underline{0.293} & 0.202/0.298 & 0.21/0.308 \\ \cline{2-7}
        % ~ & 192 & \textbf{0.211}/\textbf{0.31} & \underline{0.217}/0.313 & 0.238/0.337 & 0.227/0.321 & 0.223/\underline{0.312} \\ \cline{2-7}
        % ~ & 336 & \textbf{0.229}/\textbf{0.323} & 0.258/0.353 & 0.273/0.364 & \underline{0.256}/\underline{0.345} & 0.282/0.357 \\ \cline{2-7}
        % ~ & 720 & \textbf{0.375}/\textbf{0.444} & \underline{0.43}/\underline{0.475} & 0.455/0.49 & 0.442/0.479 & 0.606/0.561 \\ \cline{2-7}
        % ~ & Avg & \textbf{0.251}/\textbf{0.342} & \underline{0.277}/\underline{0.361} & 0.291/0.371 & 0.282/\underline{0.361} & 0.33/0.385 \\ \hline\hline
        % \multirow{5}{*}{Traffic} & 96 & \underline{0.56}/0.411 & 0.607/0.417 & \textbf{0.543}/\underline{0.408} & 0.591/0.423 & 0.577/\textbf{0.403} \\ \cline{2-7}
        % ~ & 192 & \textbf{0.575}/\underline{0.419} & 0.603/0.421 & \underline{0.594}/0.431 & 0.613/0.432 & 0.596/\textbf{0.411} \\ \cline{2-7}
        % ~ & 336 & \textbf{0.597}/\textbf{0.433} & \underline{0.63}/\underline{0.435} & 0.659/0.458 & 0.639/0.445 & 0.665/0.454 \\ \cline{2-7}
        % ~ & 720 & \underline{0.65}/\underline{0.452} & \textbf{0.643}/\textbf{0.439} & 0.69/0.49 & 0.744/0.496 & 0.802/0.501 \\ \cline{2-7}
        % ~ & Avg & \textbf{0.595}/\underline{0.429} & \underline{0.621}/\textbf{0.428} & 0.622/0.447 & 0.647/0.449 & 0.66/0.442 \\ \hline\hline
        % \multirow{5}{*}{Weather} & 96 & \textbf{0.217}/\textbf{0.268} & 0.288/0.31 & 0.252/0.288 & \underline{0.237}/0.288 & 0.249/\underline{0.285} \\ \cline{2-7}
        % ~ & 192 & \textbf{0.265}/\textbf{0.302} & 0.305/0.331 & 0.322/0.336 & 0.291/0.323 & \underline{0.277}/\underline{0.314} \\ \cline{2-7}
        % ~ & 336 & \underline{0.322}/\underline{0.342} & 0.338/0.353 & 0.346/0.358 & 0.335/0.354 & \textbf{0.311}/\textbf{0.341} \\ \cline{2-7}
        % ~ & 720 & 0.41/0.397 & \textbf{0.381}/\textbf{0.377} & 0.444/0.42 & 0.466/0.436 & \underline{0.385}/\underline{0.386} \\ \cline{2-7}
        % ~ & Avg & \textbf{0.304}/\textbf{0.327} & 0.328/0.343 & 0.341/0.351 & 0.332/0.35 & \underline{0.305}/\underline{0.331} \\ \hline\hline

        
    \end{tabular}
    }
\end{small}
\end{wraptable}


==> tex/prob.tex <==
\section{Problem Definition}
Given observed values of previous $K$ timestamps, the task of \textit{multivariate time-series forecasting} aims to predict the values for the next $H$ timestamps. That is,
\begin{equation}
\hat{\bold{x}}_{t}^i, ..., \hat{\bold{x}}_{t+H-1}^i = F(\bold{x}^i_{t-K},...,\bold{x}^i_{t-1};\mathbf{V}^i;\Phi)
\end{equation}
where $\hat{\bold{x}}_{t+i}^i, ..., \hat{\bold{x}}_{t+i+H-1}^i$ is the vector of H-step estimation from timestamp $t$ of channel $i$ among all channels of multiple features. Given the historical values $\bold{x}_{t-K}^i,...,\bold{x}_{t-1}^i$, it can be inferred by model $F$ with parameter $\Phi$ and prompt $\mathbf{V}^i$.
